The Validity of the Local Density Approximation for Smooth Short Range Interaction Potentials

In the full quantum theory, the energy of a many-body quantum system with a given one-body density is described by the Levy-Lieb functional. It is exact, but very complicated to compute. For practical computations, it is useful to introduce the Local Density Approximation which is based on the local energy of constant densities. The aim of this paper is to make a rigorous connection between the Levy-Lieb functional theory and the Local Density Approximation. Our justification is valid for fermionic systems with a general class of smooth short range interaction potentials, in the regime of slowly varying densities. We follow a general approach developed by Lewin, Lieb and Seiringer for Coulomb potential, but avoid using any special properties of the potential including the scaling property and screening effects for the localization of the energy.

==> Conclusion.tex <==
{
In this \type{} we proved the existence of a function $\elda$ which is defined as the energy of a constant density in the thermodynamic limit,
\begin{equation*}
	\elda(\rho_0) = \lim_{N \to \infty} \frac{E(\rho_0\mathds{1}_{\Omega_N} \ast \chi_{\delta_N})}{|\Omega_N|}.
\end{equation*}
There are only relatively weak assumptions on the objects involved in this definition, so it should be possible to find good numeric approximations to it.

We then used this function to prove the validity of the Local Density Approximation, namely
\begin{multline*}
	\left| E(\rho_N) - N \intR \elda(\rho(x)) \; dx \right| \\
	\leq CN^{7/15} \intR |\nabla \sqrt{\rho}(x)|^2 \; dx + CN^{13/15} \intR \left( \rho(x) + \rho(x)^2 + |\nabla \sqrt{\rho} (x)|^4 \right) \; dx
\end{multline*}
where we are taking $\rho_N(x) = \rho(N^{-1/3}x)$.

First, let us remark that our error term $N^{13/15}$ is slightly better than $N^{11/12}$ for the Coulomb interaction in \cite{Lewin_2020}. However, it is expected \cite{Kirzhnits_1957} that the next order of expansion involves at least a gradient term as correction to the kinetic energy which has order $N^{1/3}$.

One reason we are very far from this is the subadditivity estimate in Lemma \ref{lem:subadd} where we get an error of the form $\eps^{-1}D(\rho)$ which then turns into the error $\eps^{1-5/2p} \intR |\nabla \rho^\theta|^p$ in our case. Here we see why we could improve a little in comparison to the Coulomb case, we can use the boundedness of $\omega$ to estimate the direct term against the $L^2$ norm, whereas for the Coulomb interaction, one has to use the Hardy-Littlewood-Sobolev inequality with the $L^{6/5}$ norm. We see that even when we assume our interaction to be much more regular, we still only improved our error exponent from $11/12$ to $13/15$. This shows that there are certainly new ideas needed to improve the order of convergence, in particular, this is not a Coulomb specific problem.

On the other hand, we saw that the regularity of the function $\elda$ is important for the validity of the LDA. While this is easy to see for interactions with scaling properties such as Coulomb, a slightly weaker regularity still holds true if $\omega$ and $\hat{\omega}$ are radially decreasing. This allowed us to investigate the local behaviour of $\elda$ without having to compute or finding numerical approximations to it. We required $\omega$, $\hat{\omega} \in L^1$ but it seems interesting to find less restrictive assumptions such that $\elda$ still has enough regularity.

While Density Functional Theory has a long history in mathematics, physics and chemistry, mathematically rigorous justifications for it are rare. We hope that the methods and techniques used in \cite{Lewin_2020} and in this work will lead to a better understanding and verification for Density Functional Theories in the future.
}
